Multigrid methods for the Stokes problem on GPU systems

This paper presents a matrix-free multigrid method for solving the Stokes problem, discretized using $H^{\text{div}}$-conforming discontinuous Galerkin methods. We employ a Schur complement method combined with the fast diagonalization method for the efficient evaluation of the local solver within the multiplicative Schwarz smoother. This approach operates directly on both the velocity and pressure spaces, eliminating the need for a global Schur complement approximation. By leveraging the tensor product structure of Raviart-Thomas elements and an optimized, conflict-free shared memory access pattern, the matrix-free operator evaluation demonstrates excellent performance numbers, reaching over one billion degrees of freedom per second on a single NVIDIA A100 GPU. Numerical results indicate efficiency comparable to that of the three-dimensional Poisson problem.

==> tmp.tex <==
For cells of arbitrary shape, a mapping that preserves divergence is critical. The Piola transform, which maps the vector field $\hat{\boldsymbol{v}}$ under the transformation $\boldsymbol{F}_K$ to a vector field $\boldsymbol{v}$ is defined as $\boldsymbol{v}=\text{det}(\mathcal{J}_K)^{-1} \mathcal{J}_K \hat{\boldsymbol{v}}$.

Integrals required in the weak formulation from equation~\eqref{eq:weak_form} are calculated numerically in the reference space. This involves summing up evaluations of the integrands at quadrature points $\hat{\mathbf{x}}_q$, weighted by $\omega_q$, derived from the tensor product of 1D quadrature rules. For instance, the cell term $(q_h, \nabla \cdot \boldsymbol{u}_h)$ in~\eqref{eq:weak_form} is approximated as follows
\begin{equation}
    (\psi_i, \nabla \cdot \boldsymbol{u}_h)_K =  \int_{\hat{K}} \varphi_i(\hat{\mathbf{x}})
     \nabla \cdot\varphi(\hat{\mathbf{x}}) \mathrm{d}\hat{\mathbf{x}} 
      \approx  \sum_q \varphi_i(\hat{\mathbf{x}}_q) \nabla \cdot\varphi(\hat{\mathbf{x}}_q) \omega_q.
\end{equation}
Considering the linearity of the Stokes operator as formulated in~\eqref{eq:weak_form}, the integration of the equation against all test functions $\boldsymbol{v}_h$ and $q_h$ effectively translates to a matrix-vector operation. This operation takes a vector of coefficients $\begin{pmatrix}\mathbf{u} \\ p\end{pmatrix}=\begin{pmatrix}\left[\mathbf{u}_i\right] \\ \left[p_i\right]\end{pmatrix}$ from the solution field $\boldsymbol{u}_h$ and $p_h$ and returning the resulting integrals $\begin{pmatrix}\mathbf{y} \\ z\end{pmatrix}=\begin{pmatrix}\left[\mathbf{y}_i\right] \\ \left[z_i\right]\end{pmatrix}$,
\begin{equation*}
    \begin{pmatrix}\mathbf{y} \\ z\end{pmatrix}=\mathcal{A}_h\begin{pmatrix}\mathbf{u} \\ p\end{pmatrix}.
\end{equation*}





Drawing on the techniques discussed in~\cite{witte2022fast}, we explore the tensor structure of Raviart-Thomas elements, focusing here on the two-dimensional case for simplicity. Node functionals of these elements are expressed as follows:
\begin{gather*}
\begin{aligned}
    \mathcal{N}^{int}_j(\boldsymbol{v}) & = \int_K \boldsymbol{v} \cdot \boldsymbol{w}_j \,\, d\boldsymbol{x}, \qquad \boldsymbol{w}_j \in \mathbb{Q}_{k-1, k} \times \mathbb{Q}_{k, k-1}, \\
    \mathcal{N}^{\partial}_{i,j}(\boldsymbol{v}) & = \int_{F_i} \boldsymbol{v} \cdot \boldsymbol{n} q_j \,\, d\boldsymbol{s}, \qquad q_j \in \mathbb{Q}_k(F_i), \quad F_i \subset \partial K.
\end{aligned}
\end{gather*}
First, we consider \ccnote*{}{a basis} from $ \mathbb{Q}_{k-1, k} \times \mathbb{Q}_{k, k-1}$, where functions related to the first component are enumerated first, followed by those of the second component. Moment-based functionals on the unit interval are defined as:
\begin{equation}\label{eq:base_n}
    \mathcal{N}^{1D}_j(\varphi) = \int^1_0 \varphi q_j \,\, dx, \qquad q_j \in \mathcal{P}_k([0,1]),\qquad j = 0, ..., k.
\end{equation}
Further, we define another set of degrees of freedom on the unit interval, encompassing node values and moments:
\begin{gather}
\begin{aligned}
    \mathcal{M}^{1D}_0(\varphi) &= \varphi(0) \\
    \mathcal{M}^{1D}_{k+1}(\varphi) &= \varphi(1) \\
    \mathcal{M}^{1D}_j(\varphi) &= \int^1_0 \varphi q_{j} \,\, dx, \qquad q_{j} \in \mathcal{P}_{k-1}([0,1]),\qquad j = 1, ..., k.
\end{aligned}
\end{gather}
Using this notation, the \ccnote*{}{node} Raviart-Thomas functionals corresponding to the boundary $\{0\} \times [0,1]$ for $i=1$ decompose as:
\begin{equation}\label{eq:sf_bd}
    \mathcal{N}^{\partial}_{0,j}(\boldsymbol{v}) = v^{(1)}_1(0) \int^1_0 v^{(2)}_1 q_j \,\, dx = 
    \mathcal{M}^{1D}_1\otimes\mathcal{N}^{1D}_j(v^{(1)}_1\otimes v^{(2)}_1).
\end{equation}
for $q_j\in\mathcal{P}_{k}([0,1]), j=0,...,k$. For the opposite boundary $\{1\} \times [0,1]$, only $\mathcal{M}^{1D}_0$ is substituted by $\mathcal{M}^{1D}_{k+1}$. Similarly, node functionals for Raviart-Thomas elements that have a non-zero first vector component of $\boldsymbol{w}_j$ decompose into:
\begin{equation}\label{eq:sf_int}
    \mathcal{N}^{int}_{j}(\boldsymbol{v}) = \int^1_0 v^{(1)}_1 w^{(1)}_{1;i} \,\, dx_1 \int^1_0 v^{(2)}_1 w^{(2)}_{1;j} \,\, dx_2 = 
    \mathcal{M}^{1D}_{i+1}\otimes\mathcal{N}^{1D}_j(v^{(1)}_1\otimes v^{(2)}_1).
\end{equation}
for $w_{1;(i,j)}\in\mathbb{Q}_{k,k-1}, i=0,...,k-1, j=0,...,k$. Each primitive basis function’s first vector component in $\text{RT}_k$ is uniquely defined by the tensor product of these functionals. Similar decompositions apply for functionals related to the nonzero second vector component of $\boldsymbol{w}_j$ and boundaries aligned with the second coordinate, completing the basis functions’ definitions in $\text{RT}_k$. Degrees of freedom are schematically depicted in Figure~\ref{fig:RT2}. By adhering to the lexicographic ordering of $\mathcal{M}^{1D}_j$ functionals, efficient operator applications using Raviart-Thomas elements are achieved. For further insights, refer to~\cite{KronbichlerKormann19, Cui2024}
